Tensor Topic Modeling Via HOSVD

By representing documents as mixtures of topics, topic modeling has allowed the successful analysis of datasets across a wide spectrum of applications ranging from ecology to genetics. An important body of recent work has demonstrated the computational and statistical efficiency of probabilistic Latent Semantic Indexing (pLSI)-- a type of topic modeling -- in estimating both the topic matrix (corresponding to distributions over word frequencies), and the topic assignment matrix. However, these methods are not easily extendable to the incorporation of additional temporal, spatial, or document-specific information, thereby potentially neglecting useful information in the analysis of spatial or longitudinal datasets that can be represented as tensors. Consequently, in this paper, we propose using a modified higher-order singular value decomposition (HOSVD) to estimate topic models based on a Tucker decomposition, thus accommodating the complexity of tensor data. Our method exploits the strength of tensor decomposition in reducing data to lower-dimensional spaces and successfully recovers lower-rank topic and cluster structures, as well as a core tensor that highlights interactions among latent factors. We further characterize explicitly the convergence rate of our method in entry-wise $\ell_1$ norm. Experiments on synthetic data demonstrate the statistical efficiency of our method and its ability to better capture patterns across multiple dimensions. Additionally, our approach also performs well when applied to large datasets of research abstracts and in the analysis of vaginal microbiome data.

==> tex-inputs/minimax.tex <==
\section{Minimax bound}
Define the set
\begin{align*}
    \Phi^*=\left\{\begin{array}{cc}
    (A^{(1)},A^{(2)},A^{(3)}, \mathcal{G}): &\text{Assumptions \ref{ass: min singular value}-\ref{ass: min value A3} are satisfied;}\\&\min_{r\in[R]}\sum_{k\in[K^{(3)}]} A^{(3)}_{rk}\geqslant\sqrt{\frac{}{N^{(1,2)}M}}\end{array} \right\}
\end{align*}
\begin{proposition}[Lemma 12 of \cite{bing2020optimal} and Theorem 2.5 of \cite{Tsybakov2008IntroductionTN}]\label{prop:lowerbound}  Let $G=\mathcal{M}_3(\mathcal{G})$. 
Consider $(A^{(1)}_0,A^{(2)}_0,A^{(3)}_0, G_0)$, $(A^{(1)}_1,A^{(2)}_1,A^{(3)}_1, G_1)$, \dots, $(A^{(1)}_T,A^{(2)}_T,A^{(3)}_T, G_T)\in\Phi^*$. For $t=0,1,\dots, T$, let $D_t$ be the corresponding matrix $D_t=A^{(3)}_t\cdot G_t \cdot \left(A^{(1)\top}_t\otimes A^{(2)\top}_t\right)\in\mathbb{R}^{R\times N^{(1,2)}}$, each column of which is weight vector. Under model \eqref{eq: model multinominal}, let  $\mathbb{P}_0$ and $\mathbb{ P}_t$ be the probability measures associated with $D_0$ and $ D_t$, respectively. Let $\mathcal{T}_t$ be the set such that 
$$\mathcal{T}_t:=\{(r,ij)\in[R]\times [N^{(1,2)}]: D_0(r,ij)= D_t(r,ij)=0\}.$$
Let $\mathcal{T}_t^c=([R]\times [N^{(1,2)}])\backslash \mathcal{T}_t$ and
$\delta_t=\max_{(r,ij)\in \mathcal{T}_t^c}\frac{| D_0(r,ij)-D_t(r,ij)|}{D_0(r,ij)}$ for all $t\in[T]$. Let the parameter $\theta_t\in\{A^{(1)}_t,A^{(2)}_t,A^{(3)}_t, G_t\}$. Given $\theta_t$, if there exists $\epsilon_{\theta}>0$ such that
\begin{enumerate}
    \item[(i)] $\mathcal{L}(\theta_t,\theta_{t'})\geqslant C_0 \epsilon_{\theta}$ for all $0\leqslant t\neq t'\leqslant T$,
    \item[(ii)] $\delta_t< 1$
     \item[(iii)] $ M\sum_{(r,ij)\in\mathcal{T}_j^c}\frac{| D_0(r,ij)-D_t(r,ij)|^2}{D_0(r,ij)}\leqslant  \log T /16 $ for all $t\in[T]$,
\end{enumerate}
then there exists a universal constant $C>0$ such that 
$$
\inf_{\hat \theta}\sup_{(A^{(1)},A^{(2)},A^{(3)}, G)\in\Phi^*}\mathbb{P}\left(\mathcal{L}(\hat \theta, \theta)\geqslant C_0 \epsilon_{\theta}\right)\geqslant c'
$$
where for a constant $c'>0$
    
\end{proposition}
Without loss of generality, we assume that the following settings:
\begin{enumerate}
    \item $K^{(1)}K^{(2)}$ is a multiple of $K^{(3)}$, $K^{(1)}\geqslant K^{(3)}\geqslant 2$.
    \item $N^{(1)}$ is a multiple of $K^{(1)}$ and $N^{(2)}$ is a multiple of $K^{(2)}$.
    \item $K^{(a)}$ are even for all $a\in[3]$.
    
\end{enumerate}
\subsection{Lower bound on $A^{(1)}$}
\begin{lemma} Under the setting in Proposition \ref{prop:lowerbound}, if $R^2\leq N^{(1,2)}M$ we have
$$
\inf_{\hat A^{(1)}}\sup_{(A^{(1)},A^{(2)},A^{(3)}, G)\in\Phi^*}\mathbb{P}\left(\mathcal{L}(\hat A^{(1)}, A^{(1)})\geqslant C_0 \epsilon_{\theta}\right)\geqslant c'
$$
\end{lemma}
\begin{proof}
Consider the matrix $\tilde A^{(1)\top}_1$ composed of $N^{(1)}/K^{(1)}$ blocks, each of which is the identity matrix $I_{K^{(3)}}$ of size $K^{(3)}$:
$$\tilde 
 A^{(1)\top}_1=\left[\begin{array}{c|c|c|c}
I_{K^{(1)}}&I_{K^{(1)}}& \cdots &I_{K^{(1)}}
\end{array}\right] $$
We have $\sigma\left(\tilde A^{(1)\top}_1\tilde A^{(1)}_1\right)=N^{(1)}/K^{(1)}$.
Set 
$$\gamma_1=\frac{1}{K^{(3)}}$$
and define the basic matrix 
\begin{align*}
A^{(1)\top}_0:=&\tilde A_{1}^{(1)\top}+\gamma_1\left[\mathbf{0}_{K^{(1)}\times K^{(1)}}| \mathbf{1}_{K^{(1)}\times (N^{(1)}-K^{(1)})}\right]\\
&-\left[\mathbf{0}_{K^{(1)}\times K^{(1)}}| K^{(1)}\gamma_1 I_{K^{(1)}}| \cdots| K^{(1)}\gamma_1I_{K^{(1)}}\right]\\
=&\left[\begin{array}{c|c|c|c}
I_{K^{(1)}}&I_{K^{(1)}}+\gamma_1\mathbf{1}_{K^{(1)}\times K^{(1)}}& \cdots &I_{K^{(1)}}+\gamma_1\mathbf{1}_{K^{(1)}\times K^{(1)}}
\end{array}\right]
\\&-\left[\begin{array}{c|c|c|c}
\mathbf{0}_{K^{(1)}\times K^{(1)}}& K^{(1)}\gamma_1 I_{K^{(1)}}& \cdots &K^{(1)}\gamma_1I_{K^{(1)}}
\end{array} \right]\\
=&\left[\begin{array}{ccc|ccc|c}
1 & \cdots & 0 & 1-(K^{(1)}-1)\gamma_1 & \cdots & \gamma_1 & \cdots \\
\vdots & & \vdots & \gamma_1  & \ddots & \gamma_1&\cdots  \\
0 & \cdots & 1& \gamma_1 &  \cdots & 1-(K^{(1)}-1)\gamma_1 &\cdots 
\end{array}\right].
\end{align*}
with $N^{(1)}/K^{(1)}$ blocks of $K^{(1)}\times K^{(1)}$ square submatrices.
Following the same arguments in the proof of Theorem 3 in \cite{klopp2021assigning}, the Wely's inequality yields
\begin{align*}
    \lambda_1(A^{(1)}_0)\leqslant 3/2\sqrt{N^{(1)}/K^{(1)}}\quad\text{and}\quad \lambda_{K^{(1)}}(A^{(1)}_0)\geqslant 1/2\sqrt{N^{(1)}/K^{(1)}}
\end{align*}
Then we define the basic matrix for other tucker components. Let
\begin{itemize}
    \item $
G_0=\left[\tilde G_0|\tilde G_0|\cdots |\tilde G_0\right]$ where $\tilde G_0=\left[\begin{array}{c|c|c|c}
e_{1},\dots,e_1&e_{2},\dots,e_2& \cdots &e_{K^{(3)}},\dots,e_{K^{(3)}}\end{array} \right]$ is a $K^{(3)}\times K^{(2,3)}$ matrix. Let $a_1=K^{(1)}/K^{(3)}$, and thus
$G_0$ has $a_1$ number of submatrix of $\tilde G_0$. It is easy to check that $\sigma\left(G_0G_0^{\top}\right)=K^{(1,2)}/K^{(3)}
$
\item $
A^{(2)\top}_0=\left[\begin{array}{c|c|c|c}
I_{K^{(2)}}&I_{K^{(2)}}& \cdots &I_{K^{(2)}}
\end{array} \right]%\in\mathbb{R}^{K^{(2)}\times N^{(2)}}
\implies \sigma\left(A^{(2)\top}_0A^{(2)}_0\right)=N^{(2)}/K^{(2)}
$
\item Let $\alpha_3=(M-K^{(3)})/M$ and $\beta_1=\frac{K^{(3)}}{RM}$. Define $
    A^{(3)}_0:=\alpha_1\left[\begin{array}{c}
    I_{K^{(3)}}\\
     \mathbf{0}_{(R-K^{(3)})\times K^{(3)}}\end{array}\right]+\beta_1\mathbf{1}_{R\times K^{(3)}}
    %\\\left[\begin{array}{cccc}  \alpha_1+\beta_1& \beta_1 &\cdots& \beta_1\\ \beta_1&\beta_1&\cdots&\beta_1\\ \vdots&\vdots& \vdots &  \mathbf{1}_{(R-K^{(3)})\times K^{(3)}}\end{array}\right]%I_{K^{(3)}}
    %\in\mathbb{R}^{R\times K^{(3)}}
    $. This implies $ \sigma(A_0^{(3)})=\{\alpha_3,0\}+\{\beta_1\sqrt{\frac{R}{K^{(3)}}},0\}$, resulting in $\sigma_1(A_0^{(3)})\leqslant\alpha_3+\beta_1\sqrt{\frac{R}{K^{(3)}}}\leqslant 1$, and $\sigma_{K^{(3)}}(A_0^{(3)})\geqslant\alpha_3-\beta_1\sqrt{\frac{R}{K^{(3)}}}\geqslant 1/4$.
\end{itemize}
All columns of the matrices defined above sum up to 1. Notice that $f_r:=\sum_{k\in[K^{(3)}]}A_{0}^{(3)}(r,k) \geqslant 1/R$ for all $r\in[R]$. And $R\leqslant\sqrt{N^{(1,2)}M}$ implies that $f_r\geqslant \sqrt{\frac{1}{N^{(1.2)}M}}$.
Observed that all the Tucker components defined above satisfy the Assumptions \ref{ass: min singular value}, \ref{ass:identifiability}, and \ref{ass: min value A3}.
Then the matrix 
\begin{align*}
&A_0^{(1,2)\top}:=A^{(1)\top}_0\otimes A^{(2)\top}_0\\=&\left[\begin{array}{c|ccc|c}
&(1-(K^{(1)}-1)\gamma_1)A_0^{(2)\top}& \cdots& \gamma_1A_0^{(2)\top} & \cdots\\
I_{K^{(1)}}\otimes A^{(2)\top}_0&\gamma_1A_0^{(2)\top} &\cdots & \gamma_1A_0^{(2)\top}&\cdots \\
&\vdots &\ddots& \vdots&\cdots\\
&\gamma_1A_0^{(2)\top} &\cdots&(1-(K^{(1)}-1)\gamma_1)A_0^{(2)\top}&\cdots
\end{array} \right]%\in\mathbb{R}^{K^{(1,2)}\times N^{(1,2)}},
\end{align*} 
has $N^{(1)}/K^{(1)}$ blocks with columns of probability vectors. Each block of $A_0^{(1,2)\top}$ is of size $K^{(1,2)}\times K^{(1)}N^{(2)}$. And define matrix 
$W_0=G_0A^{(1,2)\top}_0\in\mathbb{R}^{K^{(3)}\times N^{(1)}N^{(2)}}$, Suppose $a_1=K^{(1)}/K^{(3)}$ where $a_1\in\mathbb{N}^+$, let $\eta_1=1-(K^{(1)}-1)\gamma_1+(a_1-1)\gamma_1$. Define the matrix $\tilde W_0\in\mathbb{R}^{K^{(3)}\times K^{(1)}N^{(2)}}$ such that
\begin{align}\label{eq: tilde W_0 in A1}
    \tilde W_0=\left[\begin{array}{cccc}
      \eta_1\mathbf{1}_{N^{(2)}}^\top& a_1\gamma_1\mathbf{1}_{N^{(2)}}^\top&\cdots  &a_1\gamma_1\mathbf{1}_{N^{(2)}}^\top\\
      a_1\gamma_1\mathbf{1}_{N^{(2)}}^\top&\eta_1\mathbf{1}_{N^{(2)}}^\top& \cdots&a_1\gamma_1\mathbf{1}_{K^{(2)}N^{(2)}}^\top\\
      \vdots&\vdots&\ddots&\vdots\\
      a_1\gamma_1\mathbf{1}_{N^{(2)}}^\top&a_1\gamma_1\mathbf{1}_{N^{(2)}}^\top&\cdots&\eta_1\mathbf{1}_{N^{(2)}}^\top
    \end{array}\right]
\end{align}
Then we have \begin{align*}
 W_0=\left[ \underbrace{I_{K^{(3)}}\otimes\mathbf{1}_{N^{(2)}}^\top,\dots,I_{K^{(3)}}\otimes\mathbf{1}_{N^{(2)}}^\top}_{\text{size of }K^{(3)}\times K^{(1)}N^{(2)}}, \tilde W_0,\dots ,\tilde W_0\right]\in\mathbb{R}^{K^{(3)}\times N^{(1)}N^{(2)}}
\end{align*}
is composed of $a_1$ number of $I_{K^{(3)}}\otimes\mathbf{1}_{N^{(2)}}^\top$ and $N^{(1)}/K^{(1)}-1$ number of $\tilde W_0$.
Each column of $W_0$ is probability vector. For simplicity of notation, we denote the submatrix of $a_1$ number of $I_{K^{(3)}}\otimes\mathbf{1}_{N^{(2)}}^\top$ as $\tilde I_1\in\mathbb{R}^{K^{(3)}\times K^{(1)}N^{(2)}}$.
Therefore, the final matrix $D_0:=A_0^{(3)} G_0\left(A_0^{(1)\top}\otimes A_0^{(2)\top}\right)$ would be
\begin{align*}
    D_0=\frac{1}{1+R-K^{(3)}}\left[\begin{array}{c|c|c|c}
    \tilde I_1 &  \tilde W_0&\cdots & \tilde W_0 \\
\mathbf{1}_{(R-K^{(3)})\times K^{(1)}N^{(2)}}^\top &\mathbf{1}_{(R-K^{(3)})\times K^{(1)}N^{(2)}}^\top  &\cdots&\mathbf{1}_{(R-K^{(3)})\times K^{(1)}N^{(2)}}^\top 
    \end{array}\right]
\end{align*}
Observed that each column of $D_0$ sums up 1, $\sigma_1(D_0)\lesssim\sqrt{N^{(1,2)}}$ and $\sigma_{K^{(3)}}(D_0)\gtrsim\sqrt{N^{(1,2)}}$.
\par Our next step is to construct $A^{(1)}_t$, for $t=1,\dots, T$. Let $d=K^{(1)}(N^{(1)}-K^{(1)})/2$ Consider the set of binary sequences $B=\{0,1\}^{d}$.
Applying the Varshamov-Gilbert bound (Lemma 2.9 in \cite{Tsybakov2008IntroductionTN}), we get that there exist $\omega^{(t)}\in B$, for $\omega^{(t)}\in\mathbb{R}^d$, $t\in[T]$ such that
$$
\|\omega^{(t)}-\omega^{(t')}\|_1=\|\omega^{(t)}-\omega^{(t')}\|^2_2\geqslant \frac{d}{8} \quad\text{for any } t\neq t', t,t'=0,1,\dots, T.
$$
with $\omega^{(0)}=\mathbf{0}_{d}$ and 
$$
\log T\geqslant \frac{\log 2}{16}(2d).
$$
We divide each $\omega^{(t)}$ 
%into $N^{(1,2)}/K^{(1,2)}$ blocks, each of them, defined as $\omega^{(t)}_j$ has dimension $K^{(3)}(K^{(1,2)}-K^{(3)})/2$. For each $t$-block, we divide it 
into $N^{(1)}-K^{(1)}$ blocks, each of that has dimension $K^{(1)}/2$. We denote the $q$- block as $\omega^{(t)}_{q}\in\mathbb{R}^{K^{(1)}/2}$. For each $q$-block, we define its augmented counterpart $\tilde \omega_{q}^{(t)}=[\omega_{q}^{(t)},-\omega_{q}^{(t)}]^\top\in\mathbb{R}^{K^{(1)}}$. 
Then, given $t\in[T]$,
consider the matrix $\Delta_t$ 
\begin{align*}   \Delta_t:=\alpha_1\left[\begin{array}{c|c|c|c|c}
        \mathbf{0}_{K^{(1)}\times K^{(1)}}  & 
         \tilde \omega_{1}^{(t)}&
         \tilde \omega_{2}^{(t)}&
         \cdots &
         \tilde \omega_{N^{(1)}-K^{(1)}}^{(t)}
    \end{array}\right]\in\mathbb{R}^{K^{(1)}\times N^{(1)}}
\end{align*}
Note that all the entries of $\Delta_t\Delta_t^\top$ are bounded in absolute value by $\alpha_1^2(N^{(1)}-K^{(1)})$. Then 
$$
\alpha_1:=c_1\sqrt{\frac{1}{M}}\implies\|\Delta_t\|\leqslant\alpha_1\sqrt{K^{(1)}(N^{(1)}-K^{(1)})}\lesssim\sqrt{N^{(1)}}
$$
Now, we define, for $t\in[T]$, 
\begin{align*}
    A^{(1)}_t=A^{(1)}_0+\Delta_t^\top
\end{align*}
Then we set $D_t:=A^{(3)}_0G_0\left(A^{(1)\top}_t\otimes A^{(2)\top}_t\right)$.
It is easy to check the data $(A^{(1)}_t,D_t)$ still belongs to the set $\Phi^*$ by the Wely's inequality.
$$
\sigma_1(A^{(1)}_t)\lesssim \sqrt{N^{(1)}/K^{(1)}}\quad \text{and}\quad \sigma_{K^{(1)}}(A^{(1)}_t)\gtrsim \sqrt{N^{(1)}/K^{(1)}}
$$
and
\begin{align*}
    D_t=\frac{1}{1+R-K^{(3)}}\left[\begin{array}{c|c|c|c}
    \tilde I_1 &  \tilde W_t&\cdots & \tilde W_t \\
\mathbf{1}_{(R-K^{(3)})\times K^{(1)}N^{(2)}}^\top &\mathbf{1}_{(R-K^{(3)})\times K^{(1)}N^{(2)}}^\top  &\cdots&\mathbf{1}_{(R-K^{(3)})\times K^{(1)}N^{(2)}}^\top 
    \end{array}\right]
\end{align*}
where $\tilde W_t$ is defined alike $\tilde W_0$ in \eqref{eq: tilde W_0 in A1} by adding the components of $\tilde \omega^{(t)}$ correspondingly.
\par Observed that
$D_0(r,ij)\in\{0,1,\gamma_1,1-(K^{(1)}-1)\gamma_1\}/(1+R-K^{(3)})$ for any $r\in[R], (i,j)\in[N^{(1)}]\times [N^{(2)}]$.  we have
$D_0(r,ij)\geqslant 1/\min_r f_r$  for all $(r,ij)\in\mathcal{T}_t^c$, where $f_r\geq\sqrt{\frac{1}{N^{(1,2)}M}}$ for all $r\in[R]$ here. We are ready to prove the conditions (i)-(iii) in Proposition \ref{prop:lowerbound}.
\begin{itemize}
    \item Proof of \ref{prop:lowerbound}(i): By the definition of $A^{(1)}_t$ and the properties of $\omega^{(t)}$, we have for any $t\neq t'$
    \begin{align*}
        \|A^{(1)}_t-A^{(1)}_{t'}\|_1&=\|\Delta_t-\Delta_{t'}\|_1=2\alpha_1\cdot\|\omega^{(t)}-\omega^{(t')}\|_1
        \\& \geqslant c_1 \sqrt{\frac{  1}{M}}\cdot K^{(1)}(N^{(1)}-K^{(1)})\gtrsim N^{(1)}\sqrt{\frac{K^{(1)}}{M}}
    \end{align*}
    \item Proof of \ref{prop:lowerbound}(ii): By setting $0<c_1\leqslant 1/N^{(1,2)}$,
    \begin{align*}
        \max_{(r,ij)\in\mathcal{T}^c}\frac{|D_t(r,ij)-D_0(r,ij)|}{D_0(r,ij)}\lesssim a_1\alpha_1\cdot \frac{1}{f_r}\leqslant 1
    \end{align*}
    Direct calculations yield that
    $$
\sum_{(r,ij)\in \mathcal{T}^c}|D_t(r,ij)-D_0(r,ij)|^2=\alpha_3^2\cdot 2\|\omega^{(t)}-\omega^{(0)}\|_1\cdot N^{(1)}/K^{(1)}\cdot N^{(2)}/K^{(2)}
    $$
    Then
    \begin{align*}
KL(\mathbb{P}_{D_t},\mathbb{ P}_{D_0})&\lesssim M\sum_{(r,ij)\in\mathcal{T}^c}\frac{|D_t(r,ij)-D_0(r,ij)|^2}{D_0(r,ij)}\\
&\lesssim M/\min_{(r,ij)\in\mathcal{T}^c} D_0(r,ij) \cdot \alpha_3^2\cdot d\cdot N^{(1,2)}/K^{(1,2)}\\
&\leqslant c_0 d\leqslant \log T/16
    \end{align*}
    by choosing the constant $c_0$ properly.
    \item Then 
   % And given that $\|A^{(1,2)}_0\|_1= N^{(1,2)}$  and $f_r\geqslant\sqrt{\frac{\log N_R}{N}}$\begin{align*}    \|A^{(1,2)}_0\|_1\|G_t-G_{t'}\|_1\geqslant \|W_t-W_{t'}\|\geqslant\sqrt{\frac{ N^{(1,2)} \min_r f_r}{M}}\\  \implies \|G_t-G_{t'}\|_1\geqslant\frac{1}{\|A^{(1,2)}_0\|_1}\cdot \sqrt{\frac{ N^{(1,2)} \min_r f_r}{M}}\geqslant\end{align*}
\end{itemize}
Then we have
\begin{align*}
    \inf_{\hat G}\sup_{G}\mathbb{P}\left(\mathcal{L}(\hat G, G)\geqslant C_0\left(\frac{1}{N^{(1,2)}M}\right)^{1/4}\right)\geqslant c^*
\end{align*}

\end{proof}
\subsection{Lower bound on $G$}
Let $\tilde I_2:=I_{K^{(2)}}+\gamma_2\mathbf{1}_{K^{(2)}\times K^{(2)}}-K^{(2)}\gamma_2I_{K^{(2)}}$ with $\gamma_2=1/(4K^{(2)})$. Consider
\begin{align*}
A^{(1)\top}_0=\left[\begin{array}{c|c|c|c}
I_{K^{(1)}}&I_{K^{(1)}}& \cdots &I_{K^{(1)}}
\end{array} \right]\quad\text{and,}\quad
A^{(2)\top}_0=\left[\begin{array}{c|c|c|c}
\tilde I_2&\tilde I_2&\cdots&\tilde I_2
\end{array} \right]
\end{align*}
we have that $\sigma\left(A^{(1)\top}_0A^{(1)}_0\right)=N^{(1)}/K^{(1)}$,  $\sigma_1\left(A^{(2)}_0\right)\leqslant3/2\sqrt{N^{(2)}/K^{(2)}}$, and $\sigma_{K^{(2)}}\left(A^{(2)}_0\right)\geqslant1/2\sqrt{N^{(2)}/K^{(2)}}$.
Define \begin{align*}
A_0^{(1,2)\top}:=A^{(1)\top}_0\otimes A^{(2)\top}_0=\left[\begin{array}{c ccc|c}
A_0^{(2)\top}& \mathbf{0}_{K^{(2)}\times N^{(2)}}&\cdots& \mathbf{0}_{K^{(2)}\times N^{(2)}} & \cdots\\
\mathbf{0}_{K^{(2)}\times N^{(2)}} &A_0^{(2)\top}&\cdots & \mathbf{0}_{K^{(2)}\times N^{(2)}} &\cdots \\
\vdots& \vdots &\ddots& \vdots&\cdots\\
\mathbf{0}_{K^{(2)}\times N^{(2)}} &\mathbf{0}_{K^{(2)}\times N^{(2)}} &\cdots&A_0^{(2)\top}&\cdots
\end{array} \right]\in\mathbb{R}^{K^{(1,2)}\times N^{(1,2)}},
\end{align*}  
which has $N^{(1)}/K^{(1)}$ blocks. Each block is a $K^{(1,2)}\times K^{(1)}N^{(2)}$ submatrix. We have $\sigma\left(A^{(1,2)\top}_0A^{(1,2)}_0\right)=N^{(1,2)}/K^{(1,2)}$. Each row of $A^{(1,2)}_0$ sums up to 1. 
%Let $\tilde I_3(\gamma_3)=I_{K^{(3)}}+\gamma_3\mathbf{1}_{K^{(3)}\times K^{(3)}}-K^{(3)}\gamma_3I_{K^{(3)}}$ with $\gamma_3=1/(4K^{(3)})$
Given the unit vector $e_i\in\mathbb{R}^{K^{(3)}}$ for all $i\in[K^{(3)}]$, let the basic $G_0=\mathcal{M}_3(\mathcal{G})\in\mathbb{R}^{K^{(3)}\times K^{(1)}K^{(2)}}$ is defined by the relation
$$G_0:=\left[\underbrace{e_1,\dots,e_1}_{K^{(2)}},\dots,\underbrace{e_{K^{(3)}},\dots,e_{K^{(3)}}}_{K^{(2)}},\underbrace{e_1,\dots,e_1}_{K^{(2)}},\dots\right]$$
%\begin{align*}G_0:=&\left[\begin{array}{c|c|c|c}\tilde I_3(\gamma_3) &\tilde I_3(\gamma_3)&\cdots&\tilde I_3(\gamma_3)\end{array}\right]\in\mathbb{R}^{K^{(3)}\times K^{(1,2)}}\\=&\left[\begin{array}{ccc|ccc|c}1-(K^{(3)}-1)\gamma_3 & \cdots & \gamma_3  & 1-(K^{(3)}-1)\gamma_3 & \cdots & \gamma_3 & \cdots \\\vdots &\ddots & \vdots & \vdots & \ddots& \vdots   \\\gamma_3 &  \cdots & 1-(K^{(3)}-1)\gamma_3& \gamma_3 &  \cdots & 1-(K^{(3)}-1)\gamma_3 &\cdots \end{array}\right],\end{align*}
Each column of $G_0$ sums up to 1.  We have that $\sigma\left(G_0G_0^{\top}\right)=K^{(1,2)}/K^{(3)}$.
%\begin{align*}   \lambda_1(G_0)\leqslant 3/2\sqrt{K^{(1,2)}/K^{(3)}}\quad\text{and}\quad \lambda_{K^{(3)}}(G_0)\geqslant 1/2\sqrt{K^{(1,2)}/K^{(3)}}\end{align*}
Given $a_1=K^{(1)}/K^{(3)}$, for $a\in[K^{(3)}]$, define matrices $ \check W_a=\left[e_{a},e_{a},\cdots e_{a}\right]\in\mathbb{R}^{K^{(3)}\times N^{(2)}}$. Let $\tilde W_0$ composed of $a_1$ sets of matrices $\{\check W_a\}_{a\in[K^{(3)}]}$, such that $\tilde W_0:=\left[\check W_1,\dots,\check W_{K^{(3)}},\dots,\check W_1,\dots,\check W_{K^{(3)}}\right]\in\mathbb{R}^{K^{(1)}\times K^{(1)}N^{(2)}}$ . Let
%$W_0=G_0A^{(1,2)\top}_0\in\mathbb{R}^{K^{(3)}\times N^{(1)}N^{(2)}}$, we then have
\begin{align*}
  W_0&=\left[\tilde W_0|\cdots|\tilde W_0\right]\in\mathbb{R}^{K^{(3)}\times N^{(1)}N^{(2)}}
\end{align*}
Each column of $W_0$ also sums up to 1. $W_0$ has $N^{(1)}/K^{(1)}$ number of $\tilde W_0$ submatrices, each of which has dimension $K^{(3)}\times  N^{(2)}K^{(1)})$. %The submatrix $\tilde W_0$ itself can also divided into $K^{(1)}$ block. Each block has $N^{(2)}/K^{(2)}$ parts, each of which has dimension $K^{(3)}\times K^{(2)}$. Let $a\in[K^{(1)}]$. For all $p\in[N^{(2)}/K^{(2)}]$, the submatrix of the $p$-part in $a$-th block of $\tilde W_0$ is $G_0(\star, (a-1)K^{(2)}:aK^{(2)})\in\mathbb{R}^{K^{(3)}\times K^{(2)}}$.
Suppose we fix $K^{(a)}$ for $a\in[3]$, we have
$$
  \sigma_1(W_0 W_0^\top)\lesssim N^{(1,2)}\quad\text{and}\quad \sigma_{K^{(3)}}(W_0 W_0^\top)\gtrsim N^{(1,2)}
$$
Let $\alpha_3=\frac{M-K^{(3)}}{M}$, and $\beta_3=\frac{K^{(3)}}{M(R-K)}$the matrix $A^{(3)}_{0}$ be
\begin{align*}
    A^{(3)}_0:=\left[\begin{array}{c}
      \alpha_3 I_{K^{(3)}}\\
      \beta_3\mathbf{1}_{(R-K^{(3)})\times K^{(3)}}
    \end{array}\right]%I_{K^{(3)}}
    \in\mathbb{R}^{R\times K^{(3)}}
\end{align*}
Each column of $A^{(3)}$ is a weight vector. $\lambda_1(A_0^{(3)})\leqslant \alpha_3+\beta_3\sqrt{\frac{R-K^{(3)}}{K^{(3)}}}\leqslant 1$, while $\lambda_{K^{(3)}}(A_0^{(3)})\geqslant \alpha_3-\beta_3\sqrt{\frac{R-K^{(3)}}{K^{(3)}}}\geqslant 1/4$. 
Observed that all the Tucker components defined above satisfy the Assumptions \ref{ass: min singular value},\ref{ass:identifiability}, and \ref{ass: min value A3}.
Finally, we define
\begin{align*}
    D_0:=
    A^{(3)}_0 W_0=\left[\begin{array}{c|c|c|c}
    \alpha_3\tilde W_0   &  \alpha_3\tilde W_0&\cdots & \alpha_3\tilde W_0 \\
\beta_3\mathbf{1}_{(R-K^{(3)})\times K^{(1)}N^{(2)}}^\top &\beta_3\mathbf{1}_{(R-K^{(3)})\times K^{(1)}N^{(2)}}^\top  &\cdots&\beta_3\mathbf{1}_{(R-K^{(3)})\times K^{(1)}N^{(2)}}^\top 
    \end{array}\right]
\end{align*}
Observed that each column of $D_0$ sums up 1, $\sigma_1(D_0)\lesssim\sqrt{N^{(1,2)}}$ and $\sigma_{K^{(3)}}(D_0)\gtrsim\sqrt{N^{(1,2)}}$.
\par Our next step is to construct $G_t$. For $t=1,\dots, T$. Let $d=K^{(1,2)}(K^{(3)}-2)/2$ Consider the set of binary sequences $B=\{0,1\}^{d}$.
Applying the Varshamov-Gilbert bound (Lemma 2.9 in \cite{Tsybakov2008IntroductionTN}), we get that there exist $\omega^{(t)}\in B$, for $\omega^{(t)}\in\mathbb{R}^d$, $t\in[T]$ such that
$$
\|\omega^{(t)}-\omega^{(t')}\|_1=\|\omega^{(t)}-\omega^{(t')}\|^2_2\geqslant \frac{d}{8} \quad\text{for any } t\neq t', t,t'=0,1,\dots, T.
$$
with $\omega^{(0)}=\mathbf{0}_{d}$ and 
$$
\log T\geqslant \frac{\log 2}{16}(2d).
$$
We divide each $\omega^{(t)}$ 
%into $N^{(1,2)}/K^{(1,2)}$ blocks, each of them, defined as $\omega^{(t)}_j$ has dimension $K^{(3)}(K^{(1,2)}-K^{(3)})/2$. For each $t$-block, we divide it 
into $K^{(1,2)}$ blocks, each of that has dimension $(K^{(3)}-2)/2$. We denote the $q$- block as $\omega^{(t)}_{q}\in\mathbb{R}^{(K^{(3)}-2)/2}$. For each $q$-block, we define its augmented counterpart $\tilde \omega_{q}^{(t)}=[\omega_{q}^{(t)},-\omega_{q}^{(t)}]^\top\in\mathbb{R}^{K^{(3)}-2}$. 
Then, given $t\in[T]$,
consider the matrix $\Delta_t\in\mathbb{R}^{K^{(3)}\times K^{(1,2)}}$ 
\begin{align*}   \Delta_t:=\alpha_3\left[\begin{array}{ccc|ccc|ccc|c}
       0& \cdots& 0 & 0&\cdots&0&
        \tilde \omega^{(t)}_{2K^{(2)}+1}(1) &\cdots &\tilde \omega^{(t)}_{3K^{(2)}}(1)  &\cdots \\
         \tilde\omega^{(t)}_1&\dots &\tilde\omega_{K^{(2)}}^{(t)} &0&\cdots&0& 0&\cdots&0&\cdots
         \\
         &&&&&&0&\cdots &0&\cdots\\
       0&\cdots &0 & \tilde\omega^{(t)}_{K^{(2)}+1}&\dots &\tilde\omega_{2K^{(2)}}^{(t)}& \tilde \omega^{(t)}_{2K^{(2)}+1}(\backslash 1) &\cdots &\tilde \omega^{(t)}_{3K^{(2)}}(\backslash 1)  &\cdots 
        \end{array}\right]
\end{align*}
where $\omega^{(t)}_{2K^{(2)}+1}(\backslash 1)\in\mathbb{R}^{K^{(3)}-3}$ contains the value in $\omega^{(t)}_{2K^{(2)}+1}$ except the first entry.
Note that all the entries of $\Delta_t\Delta_t^\top$ are bounded in absolute value by $\alpha_3^2(K^{(1,2)}-a_1K^{(3)})$, thereby yielding 
$$
\|\Delta_t\|\leqslant\alpha_3\sqrt{K^{(3)}(K^{(1,2)}-K^{(3)})}
$$
Now, we define, for $t\in[T]$, 
\begin{align*}
    G_t=G_0+\Delta_t
\end{align*}
It is easy to observe that the columns of $G_t$ are still probability vectors. Let $\alpha_3:=c_3\sqrt{\frac{1}{M}}$.
If $M\geqslant 2K^{(3)}$ and the constant $c_3$ is chosen small enough, we have $\|\Delta_t\|\lesssim \sqrt{K^{(1,2)}/K^{(3)}}$. Using the Wely's inequality again yields
$$
\sigma_1(G_t)\lesssim \sqrt{K^{(1,2)}/K^{(3)}}\quad \text{and}\quad \sigma_{K^{(3)}}(G_t)\lesssim \sqrt{K^{(1,2)}/K^{(3)}}
$$
Let 
$$W_t:=G_t A^{(1,2)\top}_0 =\left[\begin{array}{c|c|c|c}
      \tilde W_t   &  \tilde W_t&\cdots & \tilde W_t 
    \end{array}\right]\in\mathbb{R}^{K^{(3)}\times N^{(1,2)}}$$
    where $\tilde W_t$ is defined similarly to $\tilde W_0$.
    This implies each column of $W_t$ is a weight vector and $\sigma_1(W_t)\lesssim \sqrt{N^{(1,2)}} \text{ and }\sigma_{K^{(3)}}(W_t)\gtrsim \sqrt{N^{(1,2)}}$.
Similarly, we define
$D_t=A^{(3)}_0 W_t$ which has weight columns and $\sigma_1(D_t)\lesssim \sqrt{N^{(1,2)}} \text{ and }\sigma_{K^{(3)}}(D_t)\gtrsim \sqrt{N^{(1,2)}}$. Observed that
$D_0(r,ij)=\{0,1,\gamma_3,1-(K^{(3)}-1)\gamma_3\}/(1+R-K^{(3)})$ for any $r\in[R], (i,j)\in[N^{(1)}]\times [N^{(2)}]$. Then
$D_0(r,ij)\geqslant 1/\min_r f_r$ where $f_r\gtrsim\frac{1}{R}$ for all $r\in[R]$ here. %The discrepancy between $D_t$ and $D_0$ only occurs at $(K^{(1,2)}-K^{(3)})K^{(3)}\cdot K^{(3)}\cdot N^{(1,2)}/K^{(1,2)}$ where $G_0$ differs from $G_t$. 
Let $$\mathcal{T}:=\{(r,q)\in[R]\times [N^{(1,2)}]: D_0(r,q)=D_t(r,q)=0\}.$$
\begin{itemize}
    \item Proof of (H.1(a)): We have 
    \begin{align*}
        \max_{(r,ij)\in\mathcal{T}^c}\frac{|D_t(r,ij)-D_0(r,ij)|}{D_0(r,ij)}\lesssim \alpha_3\leqslant 1
    \end{align*}
    Direct calculations yield that
    $$
\sum_{(r,ij)\in \mathcal{T}^c}|D_t(r,ij)-D_0(r,ij)|^2=\alpha_3^2\cdot 2\|\omega^{(t)}-\omega^{(0)}\|_1\cdot N^{(1)}/K^{(1)}\cdot N^{(2)}/K^{(2)}
    $$
    Then
    \begin{align*}
KL(\mathbb{P}_{D_t},\mathbb{ P}_{D_0})&\lesssim M\sum_{(r,ij)\in\mathcal{T}^c}\frac{|D_t(r,ij)-D_0(r,ij)|^2}{D_0(r,ij)}\\
&\lesssim M/\min_{(r,ij)\in\mathcal{T}^c} D_0(r,ij) \cdot \alpha_3^2\cdot d\cdot N^{(1,2)}/K^{(1,2)}\\
&\leqslant c_0 d\leqslant \log T/16
    \end{align*}
    by choosing the constant $c_0$ properly.
    \item Then \begin{align*}
        \|G_t-G_{t'}\|_1&=\|\Delta_t-\Delta_{t'}\|_1\\
        &=2\alpha_3\cdot\|\omega^{(t)}-\omega^{(t')}\|_1
        \\& \geqslant c_1 \sqrt{\frac{  \min_r f_r^2}{MN^{(1,2)}}}\gtrsim\left(\frac{1}{MN^{(1,2)}}\right)^{-1/4}
    \end{align*}
   % And given that $\|A^{(1,2)}_0\|_1= N^{(1,2)}$  and $f_r\geqslant\sqrt{\frac{\log N_R}{N}}$\begin{align*}    \|A^{(1,2)}_0\|_1\|G_t-G_{t'}\|_1\geqslant \|W_t-W_{t'}\|\geqslant\sqrt{\frac{ N^{(1,2)} \min_r f_r}{M}}\\  \implies \|G_t-G_{t'}\|_1\geqslant\frac{1}{\|A^{(1,2)}_0\|_1}\cdot \sqrt{\frac{ N^{(1,2)} \min_r f_r}{M}}\geqslant\end{align*}
\end{itemize}
Then we have
\begin{align*}
    \inf_{\hat G}\sup_{G}\mathbb{P}\left(\mathcal{L}(\hat G, G)\geqslant C_0\left(\frac{1}{N^{(1,2)}M}\right)^{1/4}\right)\geqslant c^*
\end{align*}

\subsection{Lower bound of $A^{(1)}$}:
Define the basic $G_0=\mathcal{M}_3(\mathcal{G})\in\mathbb{R}^{K^{(3)}\times K^{(1)}K^{(2)}}$ is defined by the relation
\begin{align*}
G_0:=&\left[\begin{array}{c|c|c|c}
I_{K^{(3)}}&I_{K^{(3)}}+\gamma_3\mathbf{1}_{K^{(3)}\times K^{(3)}}& \cdots &I_{K^{(3)}}+\gamma_3\mathbf{1}_{K^{(3)}\times K^{(3)}}
\end{array}\right]
\\&-\left[\begin{array}{c|c|c|c}
\mathbf{0}_{K^{(3)}\times K^{(3)}}& K^{(3)}\gamma_3 I_{K^{(3)}}& \cdots &K^{(3)}\gamma_3I_{K^{(3)}}
\end{array} \right]\\
=&\left[\begin{array}{ccc|ccc|c}
1 & \cdots & 0 & 1-(K_3-1)\gamma_3 & \cdots & \gamma_3 & \cdots \\
\vdots & & \vdots & \gamma_3  & \ddots & \gamma_3&\cdots  \\
0 & \cdots & 1& \gamma_3 &  \cdots & 1-(K_3-1)\gamma_3 &\cdots 
\end{array}\right],
\end{align*}
Each column of $G_0$ sums up to 1. Following the proof in Section B.5 in \cite{klopp2021assigning}, we apply Wely's inequality to matrix $G_0$. It then yields
\begin{align*}
    \lambda_1(G_0)\leqslant 3/2\sqrt{K^{(1,2)}/K^{(3)}}\quad\text{and}\quad \lambda_{K^{(3)}}(G_0)\geqslant 1/2\sqrt{K^{(1,2)}/K^{(3)}}
\end{align*}
Let the matrix $A^{(3)}_{0}$ be
\begin{align*}
    A^{(3)}_0:=\frac{1}{1+R-K^{(3)}}\left[\begin{array}{c}
      I_{K^{(3)}}\\
      \mathbf{1}_{(R-K^{(3)})\times K^{(3)}}
    \end{array}\right] I_{K^{(3)}}\in\mathbb{R}^{R\times K^{(3)}}
\end{align*}
Finally, we define\begin{align*}\tilde D_0:=A_0^{(3)}G_0=\frac{1}{1+R-K^{(3)}}\left[\begin{array}{c}   G_0  \\   \mathbf{1}_{(R-K^{(3)})\times K^{(1,2)}}\end{array}\right]\in\mathbb{R}^{R\times K^{(1,2)}}\end{align*}It is easy to observe that each column of $\tilde D_0$ is a probability vector. Each entry of $\tilde D_0$ could be understood as $\tilde D_0(r,k^{(1)}k^{(2)})=\mathbb{P}\left(\text{word }r|\text{ group } k^{(1)}, \text{ class }k^{(2)}\right)$. The the probability measures associated with $\tilde D_0$, $\mathbb{P}_{\tilde D_0}$ is the multinomial $(M,\tilde D_0)$

\subsection{Lemma}
Note that
\begin{align*}
 D'_{ji}\log \frac{D'_{ji}}{D_{ji}}&=\sum_{k} A'_{jk} W_{ki}\log \frac{\sum_{k} A'_{jk} W_{ki}}{\sum_{k} A_{jk} W_{ki}}\\
 &\leqslant  \sum_{k} A'_{jk}W_{ki}\log\left(\frac{ A'_{jk} W_{ki}}{ A_{jk} W_{ki}}\right)
 \\&\leqslant     \sum_{k} A'_{jk}W_{ki}\log\left(\frac{ A'_{jk} }{ A_{jk}}\right)
\end{align*}
